Verifying And Interpreting Neural Networks using Finite Automata

Verifying properties and interpreting the behaviour of deep neural networks (DNN) is an important task given their ubiquitous use in applications, including safety-critical ones, and their black-box nature. We propose an automata-theoric approach to tackling problems arising in DNN analysis. We show that the input-output behaviour of a DNN can be captured precisely by a (special) weak B\"uchi automaton and we show how these can be used to address common verification and interpretation tasks of DNN like adversarial robustness or minimum sufficient reasons.

==> assets/arp_orp.tex <==
% !TEX root =  ../main.tex



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-.9,xscale=.9]
	%uncomment if require: \path (0,173); %set diagram left start at 0, and has height of 173
	
	%Straight Lines [id:da30369849577439667] 
	\draw    (316,115) -- (383,115) ;
	\draw [shift={(386,115)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
	%Shape: Rectangle [id:dp9358551127242514] 
	\draw   (140,35) -- (290,35) -- (290,155) -- (140,155) -- cycle ;
	%Shape: Rectangle [id:dp3459160303004776] 
	\draw   (410,35) -- (560,35) -- (560,155) -- (410,155) -- cycle ;
	%Shape: Circle [id:dp5989055849067555] 
	\draw   (233.91,63.24) .. controls (233.91,50.52) and (244.23,40.2) .. (256.96,40.2) .. controls (269.68,40.2) and (280,50.52) .. (280,63.24) .. controls (280,75.97) and (269.68,86.29) .. (256.96,86.29) .. controls (244.23,86.29) and (233.91,75.97) .. (233.91,63.24) -- cycle ;
	%Shape: Circle [id:dp5908633873889484] 
	\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (255.76,63.24) .. controls (255.76,63.91) and (256.29,64.44) .. (256.96,64.44) .. controls (257.62,64.44) and (258.16,63.91) .. (258.16,63.24) .. controls (258.16,62.58) and (257.62,62.04) .. (256.96,62.04) .. controls (256.29,62.04) and (255.76,62.58) .. (255.76,63.24) -- cycle ;
	%Shape: Regular Polygon [id:dp15003981090961482] 
	\draw   (214,124) -- (196.73,147.78) -- (168.77,138.69) -- (168.77,109.31) -- (196.73,100.22) -- cycle ;
	%Shape: Diamond [id:dp7140449322181326] 
	\draw   (446.58,99.4) -- (483.19,109.17) -- (466.53,143.2) -- (429.93,133.43) -- cycle ;
	%Shape: Square [id:dp43013822974061955] 
	\draw   (476.18,50.67) -- (523.17,41.85) -- (531.99,88.84) -- (485,97.65) -- cycle ;
	%Curve Lines [id:da11486205723822729] 
	\draw  [dash pattern={on 4.5pt off 4.5pt}]  (182.16,118.1) .. controls (277.38,72.23) and (388.57,197.93) .. (462.92,127.18) ;
	\draw [shift={(464.04,126.1)}, rotate = 135.49] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
	%Shape: Circle [id:dp42213572534683363] 
	\draw  [dash pattern={on 4.5pt off 4.5pt}] (487.2,76.3) .. controls (487.2,68.62) and (493.42,62.4) .. (501.1,62.4) .. controls (508.78,62.4) and (515,68.62) .. (515,76.3) .. controls (515,83.98) and (508.78,90.2) .. (501.1,90.2) .. controls (493.42,90.2) and (487.2,83.98) .. (487.2,76.3) -- cycle ;
	%Curve Lines [id:da8469346359597854] 
	\draw  [dash pattern={on 4.5pt off 4.5pt}]  (256.96,40.2) .. controls (309,33.6) and (433.4,38) .. (501.1,62.4) ;
	%Curve Lines [id:da8586936496236357] 
	\draw  [dash pattern={on 4.5pt off 4.5pt}]  (256.96,86.29) .. controls (291.8,91.6) and (439.8,104.8) .. (501.1,90.2) ;
	%Shape: Circle [id:dp08908968283186747] 
	\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (179.76,118.1) .. controls (179.76,118.76) and (180.29,119.3) .. (180.96,119.3) .. controls (181.62,119.3) and (182.16,118.76) .. (182.16,118.1) .. controls (182.16,117.44) and (181.62,116.9) .. (180.96,116.9) .. controls (180.29,116.9) and (179.76,117.44) .. (179.76,118.1) -- cycle ;
	%Shape: Circle [id:dp7923342263098943] 
	\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (464.04,126.1) .. controls (464.04,126.76) and (464.58,127.3) .. (465.24,127.3) .. controls (465.91,127.3) and (466.44,126.76) .. (466.44,126.1) .. controls (466.44,125.44) and (465.91,124.9) .. (465.24,124.9) .. controls (464.58,124.9) and (464.04,125.44) .. (464.04,126.1) -- cycle ;
	
	% Text Node
	\draw (344,97.4) node [anchor=north west][inner sep=0.75pt]    {$N$};
	% Text Node
	\draw (215.5,34.6) node [anchor=south] [inner sep=0.75pt]    {$\mathbb{R}^{m}$};
	% Text Node
	\draw (485.66,34.99) node [anchor=south] [inner sep=0.75pt]    {$\mathbb{R}^{n}$};
	% Text Node
	\draw (258.96,66.64) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {$\boldsymbol{r}$};
	% Text Node
	\draw (249.4,44.26) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {$\leq d$};
	% Text Node
	\draw (189,127.4) node [anchor=north] [inner sep=0.75pt]  [font=\tiny]  {$\varphi _{\text{in}}$};
	% Text Node
	\draw (456.56,117.9) node [anchor=south] [inner sep=0.75pt]  [font=\tiny]  {$\varphi _{\text{out}}$};
	% Text Node
	\draw (508.8,54.8) node  [font=\tiny]  {$\text{class} \ k$};
	% Text Node
	\draw (321.29,134.39) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,rotate=-19.57] [align=left] {ORP};
	% Text Node
	\draw (347,63) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {ARP};
	
	
\end{tikzpicture}


==> assets/bottom-up_algo.tex <==
% !TEX root =  ../main.tex


\begin{algorithm}
	\caption{Bottom-up procedure $\tofsa$, taking arbitrary DNN and generating an input-output equivalent \FGWNBA.}
	\label{sec:translation;algo:tofsa}
	\KwIn{DNN $N$}
	\KwOut{FSA $A \in \mathcal{A}$ as stated in Th.~\ref{sec:translation;th:tofsa_correct}}
	
	$A \gets \mathit{None}$\;
	\ForEach{layer $l_i$ with input dimension $m_i$ and output dimension $n_i$}{
		$A' \gets \mathit{None}$\;
		\ForEach{node $v$ in $l_i$}{
			\lIf{$A' = \mathit{None}$}{$A' \gets \build_\mathcal{A}(v)$}
			\lElse{$A' \gets \join(A', (1, m_i),\build_\mathcal{A}(v), (1,m_i))$}
		}
		\lIf{$i = 1$} {$A \gets A'$} 
		\Else{$A \gets \project((\join(A, (m_{i-1}+1, m_{i-1} + n_{i-1}), A_{l_i}, (1,m_i))), (m_{i-1}+1, m_{i-1} + n_{i-1}))$}
	}
	\Return A 
\end{algorithm}
\TODO{Muss an neues join,del angepasst werden. -MS}

==> assets/node_build_algo.tex <==
% !TEX root =  ../main.tex


\begin{algorithm}
	\caption{Procedure $\build$ generating
	an input-output equivalent \FGWNBA for a given DNN node.}
	\label{sec:translation;algo:node_build}
	\KwIn{Node $v$ computing $\sigma(\sum_{i=1}^{k} 
	w_i x_i + b)$}
	\KwOut{$A \in \FGWNBA$ as stated in Lem.~\ref{sec:translation;lem:node_build_correct}}
	$A \gets \mathit{None}$\;
	\lIf{$k = 1$}{
		$A \gets A_{\cdot w_1}$
	}
	\Else{
		$ A \gets \project(\join(A_+, 2, A_{\cdot w_1}, 2),2)$ \;
		\ForEach{$i$ with $2 \leq i < k$}{
			$A' \gets \project(\join(A_+, 3, A, 1), 3)$ \;
			$A \gets \project(\join(A', 2, A_{\cdot w_i}, 2),2)$		
		}
	$A \gets \project(\join(A, 1, A_{\cdot w_k}, 2), 2)$
	}
	$A \gets \project(\join(A, k+1, A_{+ b}, 1),k+1)$ \;
	\Return $\project((\join(A, k+1, A_\sigma, 1)),k+1)$ 
\end{algorithm}
\TODO{Muss an neues join un del angepasst werden. -MS}

==> assets/verification_scheme.tex <==
% !TEX root =  ../main.tex



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-.9,xscale=.9]
	%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300
	
	%Shape: Regular Polygon [id:dp8859068578088967] 
	\draw   (218,98.5) -- (193.82,131.79) -- (154.68,119.07) -- (154.68,77.93) -- (193.82,65.21) -- cycle ;
	%Straight Lines [id:da10018991795582566] 
	\draw  [dash pattern={on 0.84pt off 2.51pt}]  (329,36) -- (193.82,65.21) ;
	%Straight Lines [id:da9290938483129934] 
	\draw  [dash pattern={on 0.84pt off 2.51pt}]  (423.68,90) -- (329,36) ;
	%Straight Lines [id:da7674474939851283] 
	\draw    (276,133.5) -- (343,133.5) ;
	\draw [shift={(346,133.5)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
	%Shape: Ellipse [id:dp6314128078706298] 
	\draw   (146,218.5) .. controls (146,204.69) and (161.67,193.5) .. (181,193.5) .. controls (200.33,193.5) and (216,204.69) .. (216,218.5) .. controls (216,232.31) and (200.33,243.5) .. (181,243.5) .. controls (161.67,243.5) and (146,232.31) .. (146,218.5) -- cycle ;
	%Straight Lines [id:da8517992197821853] 
	\draw  [dash pattern={on 0.84pt off 2.51pt}]  (154.68,119.07) -- (146,218.5) ;
	%Straight Lines [id:da6674779436801697] 
	\draw  [dash pattern={on 0.84pt off 2.51pt}]  (218,98.5) -- (216,218.5) ;
	%Shape: Ellipse [id:dp9340453892036154] 
	\draw   (277,218.5) .. controls (277,204.69) and (292.67,193.5) .. (312,193.5) .. controls (331.33,193.5) and (347,204.69) .. (347,218.5) .. controls (347,232.31) and (331.33,243.5) .. (312,243.5) .. controls (292.67,243.5) and (277,232.31) .. (277,218.5) -- cycle ;
	%Straight Lines [id:da7606862222277988] 
	\draw  [dash pattern={on 0.84pt off 2.51pt}]  (276,133.5) -- (277,218.5) ;
	%Straight Lines [id:da2733560094410592] 
	\draw  [dash pattern={on 0.84pt off 2.51pt}]  (346,133.5) -- (347,218.5) ;
	%Shape: Ellipse [id:dp0837398255994748] 
	\draw   (406,220) .. controls (406,206.19) and (421.67,195) .. (441,195) .. controls (460.33,195) and (476,206.19) .. (476,220) .. controls (476,233.81) and (460.33,245) .. (441,245) .. controls (421.67,245) and (406,233.81) .. (406,220) -- cycle ;
	%Straight Lines [id:da8590944462792198] 
	\draw  [dash pattern={on 0.84pt off 2.51pt}]  (484.34,103.16) -- (476,220) ;
	%Shape: Half Frame [id:dp8928834395883389] 
	\draw   (423.68,90) -- (484.34,103.16) -- (462.88,117.56) -- (437.93,112.15) -- (432.3,138.08) -- (410,153.04) -- cycle ;
	%Straight Lines [id:da25368624903799897] 
	\draw  [dash pattern={on 0.84pt off 2.51pt}]  (410,153.04) -- (406,220) ;
	%Shape: Rectangle [id:dp02944953922955862] 
	\draw  [dash pattern={on 0.84pt off 2.51pt}] (110,190) -- (510,190) -- (510,250) -- (110,250) -- cycle ;
	%Shape: Rectangle [id:dp2058700862259064] 
	\draw   (100,50) -- (250,50) -- (250,170) -- (100,170) -- cycle ;
	%Shape: Rectangle [id:dp8778435976776504] 
	\draw   (370,50) -- (520,50) -- (520,170) -- (370,170) -- cycle ;
	
	% Text Node
	\draw (329,32.6) node [anchor=south] [inner sep=0.75pt]    {$P$};
	% Text Node
	\draw (304,115.9) node [anchor=north west][inner sep=0.75pt]    {$N$};
	% Text Node
	\draw (175.5,47.6) node [anchor=south] [inner sep=0.75pt]    {$\mathbb{R}^{m}$};
	% Text Node
	\draw (438,32.4) node [anchor=north west][inner sep=0.75pt]    {$\mathbb{R}^{n}$};
	% Text Node
	\draw (183,98.5) node  [font=\small] [align=left] {in};
	% Text Node
	\draw (436.57,112.71) node [anchor=south] [inner sep=0.75pt]  [font=\small] [align=left] {out};
	% Text Node
	\draw (181,218.5) node  [font=\small]  {$A_{\text{in}}$};
	% Text Node
	\draw (312,218.5) node  [font=\small]  {$A_{\text{N}}$};
	% Text Node
	\draw (441,220) node  [font=\small]  {$A_{\text{out}}$};
	% Text Node
	\draw (310,256.5) node [anchor=north] [inner sep=0.75pt]  [font=\tiny] [align=left] {DO: emptyness, inclusion, ...};
	% Text Node
	\draw (100,236) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,rotate=-270] [align=left] {combine};
	
	
\end{tikzpicture}


==> sections/interpretability.tex <==
% !TEX root =  ../main.tex

In previous sections, the translation from DNN to automata is carried out using B\"uchi automata, 
in particular the subclass \FGWNBA. The reason for this is that infinite words are the most natural way to 
represent real numbers (and the eventually-always weak acceptance condition suffices for the constructions used here). 
%and the representation over the alphabet $\Sigma$ chosen here is also a natural one. 
Clearly, the general framework is not bound to the use of \FGWNBA. Any class of (finite-state) automata that can 
recognise relations of (encoded) real numbers, and which is closed under the constructions formulated in the lemmas above,
is also usable for DNN analysis tasks like the ones presented in Sect.~\ref{sec:verification}. 
One such example is the class of nondeterministic finite automata (NFA) over \emph{finite} words. 
Clearly, for cardinality reasons alone their inputs cannot represent all real numbers. Still,
the constructions laid out in the lemmas above are available for NFA as well, and minimisation for NFA is typically more
efficient in practice than it is for NBA. Hence, it is tempting to use NFA to analyse DNN, at the expense of a
less precise analysis. This can be seen as an abstraction mapping real numbers to their nearest integer for instance.

We present a proof-of-concept implementation, translating so called \textit{Binarized Neural Networks (BNN)} over $\Ints$, into 
input-output equivalent NFA. The BNN model \cite{HubaraCSEB16} evolved as a simple but powerful neural network model,
defined similar to DNN but with weights and bias restricted to $+1$ and $-1$.
It was shown, that this restriction nearly achieves state-of-the-art performances in comparison to the standard DNN
\cite{HCSEB_bnnperform}.

\subsubsection*{The Implementation.}
The code is written in Python.\footnote{Available via \url{https://github.com/marcosaelzer/NN2NFA}}
The construction of an NFA $\Aut{A}_N$ for a given DNN follows the inductive construction described in Sect.~\ref{sec:translation}
but the automata are always built over a minimal alphabet. For example, $\Aut{A}^k_{j=\mathsf{mult}(c,i)}$ is built over
two instead of $k$ tracks. This requires a little bit more bookkeeping when conjoining automata but it reduces the numbers
of their transitions. It would also allow numbers to be read from the least to the highest significant bit which might make 
alternative constructions conceptually simpler. Moreover, we employ the following optimisations.

\emph{Symbolic representations of transition labels.} Consider the automata for addition %$\Aut{A}^k_{j=\mathsf{add}(i_1,\ldots,i_n)}$ 
(see Fig.~\ref{fig:addition}). It is notable that transitions are invariant under permutations of the labels in tracks $i_1,\ldots,i_n$.
This is not surprising as addition is commutative. Consequently, the transition labels in these automata can be stored symbolically
as a pair $(r,n)$ with $r \in \{0,1\}$ representing the resulting bit in the addition, and $n \in \Nats$ representing
the number of $1$-bits in the tracks to be added up. Note that each such pair represent exponentially (in $k$) many transition labels.
%s e without altering the acceptance of the word, 
%	for example see Fig.~\ref{fig:addition}. 
%	Thus, only the amount of positive and negative bits in the input tapes determines the output bit and 
%	transition in the automaton. 
%	Therefore, we can represent non-sign and non-dot transitions by $(i,j,b)$ where $i$ is the number of
%	positive bits and $j$ the number of negative bits in the input and $b$ is the output bit. We use this
%	representation in the construction, which dramatically reduces the number of transitions in intermediate
%	steps.

\textit{Direct multiplication.} Instead of using iterated addition, automata for multiplication by a constant
	can be constructed directly. $\Aut{A}^k_{j=\mathsf{mult}(c,i)}$ with $c = \frac{n}{d}$ simply needs to compare the respective
	number of bits obtained from the tracks and save amount of carry bits that need to be the column of bits immediately following, i.e.\
	with the next lesser significance. Due to the way carry overflow works, such an automaton is of the same size as the one from
	Lemma~\ref{lem:const_mult}, but it can be constructed directly and is automatically deterministic and minimal.

\textit{Minimisation.} After each construction that may create a non-minimal automaton, explicit minimisation is employed.
Since NFA minimisation is PSPACE-hard in general, we use bisimulation quotienting instead. It may not produce minimal automata but it can be done in low polynomial time \cite{PT87}, and it typically yields good results in practice \cite{HOGBERG20093539}. 

%As mentioned above, the construction of $\Aut{A}_N$ follows the bottom-up approach described 
%	in Sect.~\ref{sec:translation}, namely that we build an automaton for each node, join them to get one for each layer and join these to get $\Aut{A}_N$.
%	In these intermediate steps, we can exploit the fact that our construction is based on NFA and use minimization to reduce the size of the generated 
%	automata. In particular, ... \TODO{\@ML Ich weiß garnicht genau was ihr da jetzt für ne Minimierung benutzt. Bisimulation? Wäre gut wenn du oder @EA das
%	mal kurz fertig schreibt.}

\begin{figure}[t]
	\begin{center}
		\includegraphics[width=\textwidth]{assets/impl_test_results}
	\end{center}
	\caption{
		Left chart: logarithmic scaled buildtime, number of nodes and number of transitions of the NFA resulting from translating randomly generated $\text{BNN}_\text{fix}$ with increasing number of layers, from 1 to 5. 
		Right chart: percentage of state set size reduction due to minimisations on 5
		randomly generated $\text{BNN}_\text{fix}$ each with 4 layers.}
	\label{fig:implementation_benchmark_1}
\end{figure}

\subsubsection{Benchmarks.}
We use semi-randomly generated BNN: the input size is 1, the output size
of the BNN is 1 and all layers in between consist of 2 nodes. We denote such
BNN with $\text{BNN}_\text{fix}$.
The parameters (weights and bias) of the considered $\text{BNN}_\text{fix}$ 
were chosen uniformly from $\{-1,1\}$.  
The benchmarks were computed on an Apple M1 Pro CPU with 32GB
RAM.
In the first part, we run our translation without intermediate minimization steps 
for $\text{BNN}_\text{fix}$ as specified above with 1 to 5 layers. 
The results are presented in the left chart of Fig.~\ref{fig:implementation_benchmark_1}.
The number of layers is plotted on the horizontal axis and the runtime, number of states/transitions on the two
logarithmically scaled vertical axis. The exponential blowup is
clearly indicated by the linear interpolations of the three data
series, even for these relatively shallow $\text{BNN}_\text{fix}$. The fluctuations 
are due to the varying amount of $-1$ and $1$ parameters.
However, in the right chart of Fig.~\ref{fig:implementation_benchmark_1}
we see the effect of our minimization. We considered 5 randomly 
generated $\text{BNN}_\text{fix}$ 
with 4 layers. The chart depicts the percentage of reduction of the state set due to minimisation. 
As we can see the state size reduction ranges  between 80 and >90 \%. This strongly indicates
that efficient minimization techniques are crucial for the practicability of a DNN to finite automata 
translation. 









